Scalable tensor methods for nonuniform hypergraphs

While multilinear algebra appears natural for studying the multiway interactions modeled by hypergraphs, tensor methods for general hypergraphs have been stymied by theoretical and practical barriers. A recently proposed adjacency tensor is applicable to nonuniform hypergraphs, but is prohibitively costly to form and analyze in practice. We develop tensor times same vector (TTSV) algorithms for this tensor which improve complexity from $O(n^r)$ to a low-degree polynomial in $r$, where $n$ is the number of vertices and $r$ is the maximum hyperedge size. Our algorithms are implicit, avoiding formation of the order $r$ adjacency tensor. We demonstrate the flexibility and utility of our approach in practice by developing tensor-based hypergraph centrality and clustering algorithms. We also show these tensor measures offer complementary information to analogous graph-reduction approaches on data, and are also able to detect higher-order structure that many existing matrix-based approaches provably cannot.

==> clustering-contact.tex <==
\subsection{Clustering}

In addition to centrality, our implicit TTSV algorithms also find application in a variety of clustering algorithms. One popular blueprint is use an embedding of the tensor as features for a clustering algorithm such as $k$-means. Following this approach, we aim to embed the hypergraph adjacency tensor $\A$ in $\R^{n\times q}$, where $q$ is the target embedding dimension, so that each node is represented by a $q$-dimensional vector. We perform the embedding by finding a symmetric CP-decomposition~\cite{kolda2015numerical,hitchcock1927expression} of $\A$, meaning we seek an $n\times q$ matrix $\Mx{E}$ and a vector $\Vc{\lambda}\in \R^q$ such that the tensor norm given by 

\begin{equation}f(\Vc{\lambda},\Mx{E})=||\A-\T{X}||\mbox{ with }\T{X}=\sum_{j=1}^{q}\Vc{\lambda}_j\Mx{E}_j^{\otimes r}\label{eqn:objective}\end{equation}

is minimized, where $\Mx{E}=[\Mx{E}_1 \Mx{E}_2 \cdots \Mx{E}_q]$ and $\Mx{E}_j^{\otimes r}$ is the $r$-way tensor outer product of $\Mx{E}_j$ with itself. To optimize Equation~\ref{eqn:objective}, we employ a standard first-order optimization scheme and utilize the  closed-form expressions \cite{kolda2015numerical} for the gradients
\begin{align*}
\frac{\partial f}{\partial \Vc{\lambda}_j} &= -2\left[\A\Mx{E}_j^r-\sum_{k=1}^q\Vc{\lambda}_k\langle \Mx{E}_j,\Mx{E}_k\rangle ^r\right],\\
\frac{\partial f}{\partial \Mx{E}_j} &= -2d\Vc{\lambda}_j\left[\A\Mx{E}_j^{r-1}-\sum_{k=1}^q\Vc{\lambda}_k\langle \Mx{E}_j,\Mx{E}_k\rangle ^{r-1}\Mx{E}_k\right],
\end{align*}
where $\langle \Mx{E}_j,\Mx{E}_k\rangle=\Mx{E}_j^T\Mx{E}_k$, $\A\Mx{E}_j^r=\sum_{i_1=1}^n\cdots\sum_{i_r=1}^n\A_{i_1,\dots,i_r}\prod_{k=1}^r\Mx{E}_{j_{i_k}}$ is the tensor times same vector operation (TTSV) which results in a scalar, and $\A\Mx{E}_j^{r-1}\in\R^n$ is the TTSV1 operation given by 
\[
\left[\A\Mx{E}_j^{r-1}\right]_{i_1}=\sum_{i_2=1}^n\cdots\sum_{i_r=1}^n\A_{i_1,\dots,i_r}\prod_{k=2}^r\Mx{E}_{j_{i_k}}.
\]
Note the TTSV value is obtained from the TTSV1 vector simply by taking an inner product with $\Mx{E}_j.$ In the first order scheme, computing $f$ and its derivatives requires $f$ explicitly requires $O(qn^r)$ time, but we use our implicit TTSV1 algorithm, together with the gradient computation approach outlined in~\cite{sherman2020estimating}, to cut this time down to $O(\text{TTSV1}+ nq^2)$, where $O(\text{TTSV1})$ is the worst-case runtime of Alg.~\ref{alg:TTSV1gen}. After obtaining this CP decomposition for $\A$, the resulting embedding $E\in\R^{n\times q}$ may be used as features for a standard $k$-means clustering algorithm~\cite{hartigan1979algorithm} where $k$ is the desired number of clusters. 
%In practice, the value of $k$ is chosen to correspond to the number of ground truth clusters whenever such information is available. The pipeline is presented in Figure~\ref{fig:clustering}. 
Beyond just $k$-means, the aforementioned embedding method is compatible with any metric-space clustering framework. 
\begin{figure}
    \centering
    \begin{tabular}{cc}
        \subfloat[t-SNE of Zhou laplacian embedding (a) and of the tensor embedding (b) for contact-high-school \label{fig:tsne-contact-high-school}]{\includegraphics[width=0.23\linewidth]{figs/contact-high-school-laplacian.pdf}\includegraphics[width=0.23\linewidth]{figs/contact-high-school.pdf}} &  \subfloat[t-SNE of Zhou laplacian embedding (left) and of the tensor embedding (right) for contact-primary-school \label{fig:tsne-contact-primary-school}]{\includegraphics[width=0.23\linewidth]{figs/contact-primary-school-laplacian.pdf}\includegraphics[width=0.23\linewidth]{figs/contact-primary-school.pdf}}
    \end{tabular}
    \caption{Comparison of matrix~\cite{zhou2006learning} to tensor embedding of contact-high-school (left) and contact-primary-school (right).}
    \label{fig:global_measures}
\end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width = 0.49\textwidth]{figs/contact-primary-school.pdf}
%     \includegraphics[width = 0.49\textwidth]{figs/contact-high-school.pdf}
%     \caption{t-SNE visualization of the tensor embedding for the contact-primary and contact-high-school dataset. \sga{What if you did t-SNE plot of clustering based on the clique expansion? Would the clusters not be as well separated?}} %We observe that the clusters are well-separated.}
%     \label{fig:tsne}
% \end{figure}

We now apply the aforementioned clustering approach to two hypergraph datasets from Table \ref{tab:allexp1}: contact-primary and contact-high-school. These are both proximity datasets where hyperedges connect together students (nodes) who came into close proximity with each other in a certain timeframe. These datasets benefit from having ground truth community labels, and we use these labels to color the embedding of each node. contact-high-school has 9 ground-truth clusters while contact-primary has 10 -- these numbers correspond to the number of classrooms in the schools where proximity measurements used to constrict these hypergraphs were taken. Figures~\ref{fig:tsne-contact-high-school} and~\ref{fig:tsne-contact-primary-school} present t-SNE~\cite{van2008visualizing} plots visualizing embeddings of these datasets. The left of each figure shows a visualization of a matrix-based embedding~\cite{zhou2006learning}, while the right shows the same using our tensor approach. That we observe well-separated clusters, provides qualitative evidence that the tensor embedding of $\A$ is able to distinguish communities. In fact, our tensor-based approach leads to better cluster separation in contact-high-school.
% We demonstrate that our approach is able to detect community structure in the t-SNE plots below. Note that the clusters are well-separated, implying a good embedding to distinguish communities.




% \begin{figure}[h]
%     \centering
%     \scalebox{0.80}{\input{ttsv.tex}}
%     \caption{A graphical representation of TTSV for an order 3 tensor $A$.}
%     \label{fig:ttsv}
% \end{figure}


% While we employ $k$-means to perform the clustering, our embedding method is compatible with any metric-space clustering framework.
% \begin{figure}[h]
%     \centering
%     \scalebox{0.80}{\input{clustering.tex}}
%     \caption{A visualization of our clustering framework for nonuniform hypergraphs.}
%     \label{fig:clustering}
% \end{figure}

% \newpage


% \begin{figure}[h]
%     \centering
%     \resizebox{\columnwidth}{!}{\input{centrality.tex}}
%     \caption{A visualization of our centrality framework for nonuniform hypergraphs. \sga{Very nice figure idea, but should be redone to fix several cosmetic issues: (1) equations should be centered and either all above or all below the arrows, (2) consider shortening the names to acroymns (e.g. Z-eigen ventrality is just ZEC), (3) use tensor font for $\A$, (4) TTSVOB1 should just be TTSV1, consistent with rest of paper  } \sga{Also, I am confused here that this diagram shows us forming the banerjee tensor. I thought the whole point was we don't ``encode as a tensor" and instead do implicit TTSV}}
%     \label{fig:centrality}
% \end{figure}




% \begin{algorithm}[H]
% % \SetLine
% \SetKwRepeat{Repeat}{repeat}{until}
% \KwData{rank $r$ hypergraph $H=(V,E)$, tolerance $\tau$, step size $h$}
% \KwResult{Z-eigenvector centrality, $\Vc{x}$}
% $\Vc{y}=\frac{1}{|V|} \Vc{1}$\;

% \Repeat{$\frac{\max \Vc{g} - \min \Vc{g}}{\min \Vc{g}}<\tau$}{
% $\Vc{d} = \mbox{dominant eigenvector of TTSV2}((V,E),\Vc{y})$\;

% $\Vc{x} = \Vc{y}+h\cdot(\Vc{d}-\Vc{y})$\;

% $\Vc{g}=\Vc{x}\oslash \Vc{y}, \ \Vc{y} = \Vc{x}$\;
% }
% \Return{$\Vc{x}$}
% \caption{BG algorithm for computing Z-eigenvector centrality}
% \end{algorithm}

% \xhdr{Scalable generalized H-eigenvector centrality}

% The NQI power-like algorithm commonly used to compute H-eigenvector centrality relies on TTSV1 as the workhorse for each iteration~\cite{ng2010finding}. The algorithm is presented below.

% \begin{algorithm}[H]
% % \SetLine
% \KwData{rank $r$ hypergraph $H=(V,E)$, tolerance $\tau$}
% \KwResult{H-eigenvector centrality, \Vc{x}}
% $\Vc{y}=\frac{1}{|V|} \Vc{1}$\;

% $\Vc{z}=$ TTSV1($H,\Vc{y}$)\;

% \Repeat{$\lambda_{\max} -\lambda_{\min} < \tau$}
% {
% $\Vc{x}=\Vc{z}^{\nicefrac{1}{m-1}} / ||\Vc{z}^{\nicefrac{1}{m-1}}||_1$\;

% $\Vc{z}=$ TTSV1($H,\Vc{x}$)\;

% $\lambda_{\min}, \ \lambda_{\max} = \min{(\Vc{z} \oslash \Vc{x}^{m-1})}, \ \max{(\Vc{z} \oslash \Vc{x}^{m-1})}$
% }

% %converged = false\;

% % \For{$k$ in 0:iterations}{
% % $x_{k+1}=y_{k}^{1/(m-1)}/||y_{k}^{1/(m-1)}||_1$\;
% % $y_{k+1}=$ TTSV1($A,x^{k+1}$)\;
% % $\underline{\lambda}_{k+1}=\min_i\frac{[y_{k+1}]_i}{[x_{k+1}]_{i}^{m-1}}$\Comment{Compute lower estimate of eigenvalue}\;
% % $\bar{\lambda}_{k+1}=\max_i\frac{[y_{k+1}]_i}{[x_{k+1}]_{i}^{m-1}}$\Comment{Compute upper estimate of eigenvalue}\;
% % converged = $\bar{\lambda}_{k+1}-\underline{\lambda}_{k+1} <$ tolerance\;
% % \If{\mbox{converged}}{break}
% % }
% \Return{$\Vc{x}$}
% \caption{NQI algorithm for computing H-eigenvector centrality}
% \end{algorithm}
% \subsection{Clique expansion eigenvector centrality of general (weighted) hypergraphs}
% This centrality measure was first introduced in~\cite{benson2019three} in the uniform case. The nonuniform case was first presented in~\cite{amburg2021planted}, but was not analyzed there as it acted solely as a baseline to compare against. Here, we present the details of clique eigenvector centrality and analyze it. In particular, we show that it is stable and continuous in the notion of~\cite{segarra2015stability} as we change the weighting scheme. Furthermore, we show that the measure changes little when a hyperedge is added to ``unimportant'' nodes. Even when it is added to important nodes, we obtain a bound for the change in terms of their importances. These results are afforded by being able to apply the richly developed matrix eigenvector theory, which is either not possible or has not yet been developed in the case of matrices.

% \xhdr{Clique expansion eigevector centrality} Given a hypergraph $G,$ define its $n\times m$ weighted incidence matrix $I$ by writing $I_{v,e}=w_e$ if node $v$ appears in edge $e$ and $0$ otherwise. It is well-known that the clique adjacency matrix $$W=\sqrt{I}\sqrt{I^T}-D_V$$ where $D_V$ is a diagonal matrix with the weighted node degrees on its main diagonal corresponds to the adjacency matrix of a ``projected graph'' where $$W_{i,j}= \mbox{\# of times nodes $i$ and $j$ appear together in a hyperedge weighted by hyperedge weight}$$
% and the square root is taken componentwise.
% The clique eigenvector centrality vector $c$ is then the leading eigenvector of the system $$Wc=\lambda c.$$ In this formulation, a node is central if its neighbors are central in the weighted projected clique graph.

% \xhdr{Clique expansion eigenvector centrality is stable and continuous} Let us define the notions of stability and continuity that we use here.
% \begin{definition}
% A centrality measure $C$ is \textbf{stable} if given a vertex set $V$ and a set of hyperedges $E$ defined on it, given any two weighted hypergraphs $G$ and $H$ with those vertex and edge sets, we have $$|C^G(v)-C^H(v)|\leq K_G d(G,H)$$ for every node $v\in v$, where $C^G(v)$ is the centrality of node $v$ in G, $C^H(v)$ is its centrality in $H$, $K_G$ is a constand that depends on $G$, and $d(G,H)=\sum_{u,v}|W_G[u,v]-W_H[u,v]|$ is the weighted ``distance'' between the hypergraphs.

% \end{definition}

% \begin{definition}

% Given a weighted hypergraph $G$ on node set $V$ and edge set $E$ that has a projected graph incidence matrix $W_G$, define another matrix $W_\epsilon$ that has the same zero structure as $W_G$ so that $W_G+W_{\epsilon}\geq 0$, consider the weighted hypergraph $H$ on $(V,E)$ such that its projected graph incidence matrix is $W_G+W_\epsilon$. Then $C$ is a \textbf{continuous} centrality if $C^H(v)\to C^G(v)$ as $||W_\epsilon||_1\to 0$ for every node $v\in V$.

% \end{definition}

% The stability and continuity of clique expansion eigenvector centrality follows from the following theorem.

% \begin{theorem}

% Clique expansion eigenvector centrality for general hypergraphs is stable and continuous.
% \end{theorem}

% \begin{proof}
% Given two weighed hypergraphs $G$ and $H$ that are defined on the same node set, we know that changing the hyperedge weights will not affect the zero pattern of the corresponding projected graph adjacency matrices $W_G$ and $W_H$. By Proposition 4 in~\cite{segarra2015stability} the clique eigenvector centrality is stable, and by Proposition 6 it must also be continuous.

% \end{proof}

% % \xhdr{Perturbations in the unweighted case}
% % We want to quantify by how much any given component of the clique eigenvector centrality can change if we introduce one hyperedge. The following theorem will allow us to make these conclusions.
% % \begin{theorem}\label{thm:bound}
% % Given an unweighted hypergraph $G=(V,E),$ suppose that its clique expansion eigenvector centrality is $v$ with corresponding leading eigenvalue $\lambda$. If we include an additional hyperedge $h=\{i_1,\dots,i_k\}$ then the new eigenvector centrality vector $v'$ satisfies  $$\min_{s=\pm 1}||v-v'||_\infty\leq 8||v||_\infty\frac{\eta^2}{\lambda^2}+2\omega\frac{\mu}{\lambda}+4\omega\sqrt{k-1}\frac{\eta}{\lambda^2}$$
% % where $\eta^2=\sum_{l=1}^{k}\left[\sum_{j\in h\setminus\{i_l\}}v_j\right]^2,$ $\mu=\max_{l=1,\dots,k}\sum_{j\in h\setminus\{i_l\}}v_j$, and $\omega=||I-vv^T||_\infty$.
% % \end{theorem}
% % \begin{proof}

% % Suppose that the clique expansion adjacency matrix of the hyperedge is $A$. Then by the main theorem in~\cite{damle2020uniform} we know that $$\min_{s=\pm 1}||v-v'||_\infty\leq 8||v||_\infty\frac{||Av||_2^2}{\lambda^2}+2\omega \frac{||Av||_\infty}{\lambda}+4\frac{||Av||_2}{\lambda^2}\max_i||A[i,:]||_2$$
% % so it remains to show that $||Av||_2=\eta$ and $||Av||_\infty=\mu$ and $\max_i||A[i,:]||_2=\sqrt{k-1}$. The last statement follows since each vertex in the clique subgraph corresponding to $A$ has degree $(k-1)$. The first and middle statements follow since $A[l,j]v_j$ is nonzero and equal to $v_j$ precisely at indexes $j\in h\setminus \{i_l\}$ for every $l\in\{1,\dots,k\}$. This concludes the proof.
% % \end{proof}

% % The formulation in the preceeding theorem allows us to get an intuition for what factors will make the increase potentially large. The following corollary shows that The componentwise change is greatest when the nodes in $h$ are ``important'' in terms of the values in $v$ and least when the nodes are not important.

% % \begin{coro}

% % The upper bound in Theorem~\ref{thm:bound} is maximized when the nodes in $h$ correspond to the indexes of components in $v$ having the greatest values while it is minimized if they correspond to components having the smallest values in $v$.
% % \end{coro}

% % \begin{proof}

% % This is clear since $\eta$ is a sum of squares of sums of the positive components of $v$ corresponding to the nodes in $h$ while $\mu$ is a maximum over sums of those same components.
% % \end{proof}

% \subsection{Tensor eigenvector centrality detects higher-order information}
% Here, we present a case study on a synthetic dataset that demonstrates that $H$- and $Z$- tensor eigenvectors are able to distinguish higher-order patterns that standard graph projection methods are incapable of detecting. In particular, we consider two hypergraphs, $G_A$ and $G_B$ seen in the figure below. $G_A$ and $G_B$ both have the same clique expansions, and the clique expansions of their line graphs are also the same. In particular, if $A$ is the node-hyperedge incidence matrix of $G_A$ and $B$ is the same for $G_B,$ then $W=A^TA=B^TB$ and $W'=AA^T=BB^T.$ These kinds of hypergraphs are refered to as gram mates~\cite{everett2013dual,kirkland2018two,kim2022gram}. Since all graph projection approaches work on either $W$ or $W'$, the two hypergraphs are rendered indistinguishable under this approach, meaning, foe example, the resulting clique expansion eigenvector centralities are the same. However, we show that the corresponding $H$- and $Z$-eigenvector centralities \textit{do} distinguish the the two hypergraphs, producing meaningfully different centrality vectors.


% \section{Experiments}
% Here, we conduct two suites of experiments that demonstrate the usefulness of our methods and their superiority to baselines. The first suite shows that our methods perform orders of magnitude faster on both synthetic and real-life datasets. The second suite showcases results for two applications: clustering and centrality of the underlying hypergraph. In particular, we demonstrate the superiority of our clustering scheme to other tensor-based methods, and highlight the effectiveness of our tensor-eigenvector-based centralities in finding meaningfully-different rankings of nodes.


% \subsection{Performance on random hypergraphs}

% \xhdr{A hypergraph stochastic block model}
% Here, we describe a simple hypergraph generation scheme which we use to test the ability of our method to recover ground truth assignment in the stochastic setting, with the presence of noise. We randomly partition $n$ nodes into $k$ clusters. We form hyperedges on nodes within clusters with probability $q$. We form edges across clusters with probability $p$. The maximum hyperedge size $r$ is also taken as a parameter. If we want, we can choose $q=1-p$ to reduce the dimensionality.

% \subsection{Tensor operation run times}
% Here, we present runtime experiments on synthetic and real-life hypergraphs demonstrating the superiority of our approach to existing methods and baselines.
% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{figs/ttsv1-times}
%     \caption{Speedup factors of the generating-function-based algorithm for TTSV1 vs. the combinations-based, naive baseline, and explicit sparse tensor baseline. Missing times indicate that a) the combinations-based or naive baseline algorithms timed out after 1 hour or b) the explicit tensor baseline algorithm forced an out-of-memory error.}
%     \label{fig:ttsv1_time}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{figs/ttsv2-times}
%     \caption{Speedup factors of the generating-function-based algorithm for TTSV2 vs. the combinations-based, naive baseline, and explicit sparse tensor baseline. Missing times indicate that a) the combinations-based or naive baseline algorithms timed out after 1 hour or b) the explicit tensor baseline algorithm forced an out-of-memory error.}
%     \label{fig:ttsv1_time}
% \end{figure}
% \subsection{Applications}

% \subsubsection{Clustering}
% \xhdr{Results on real-life datasets}
% We test the performance of the algorithm by comparing against a spectral method followed by $k$-means on the projected graph corresponding to the hypergraph. We test performance on two real-world datasets:

% 1) Yelp Madison~\cite{amburg2020hypergraph}, where hyperedges connect reviewers who wrote reviews of restaurants of a given cuisine over the course of a month and node labels correspond to the majority review category; 2) Amazon blues~\cite{amburg2020hypergraph}, where hyperedges connect reviewers of products who wrote reviews in a given subgenre of vinyl blues records over the course of a month and node labels correspond to the majority review category.
% %and 3) SPECT~\cite{zhen2021community}, where hyperedges connect patients who share the same categorical features and node labels correspond to the presence or absence of a cardiovascular disease.
% We use the scaled hamming distance~\cite{zhen2021community} between the ground truth node labels and the clustering to compare across methods, the performance of which is noted in Table~\ref{tab:results}.

% \begin{table}[h]
%     \centering
%     % \begin{tabular}{c|ccc}
%     %      dataset & $r\leq$&tensor error  &projected error\\
%     %      \hline
%     %     Yelp Madison & 3&  \textbf{0.138}& 0.144\\
%     %     Amazon blues & 3 & \textbf{0.284}& 0.321
        
%     % \end{tabular}
%     \begin{tabular}{c|ccc}
%          dataset & $r\leq$&tensor NMI  &projected NMI\\
%          \hline
%         madison-restaurant-reviews & 3&  \textbf{0.166}& 0.095\\
%         vegas-bars-reviews & 5&  \textbf{0.235}& 0.092\\
%         contact-primary-school & 3 & \textbf{0.672} & 0.582
%         % Amazon blues & 3 & \textbf{0.284}& 0.321
        
%     \end{tabular}

%     \caption{Performance of the tensor-based algorithm vs. a spectral clustering baseline. We report the filtering parameter $r$ that resulted in the best performance increase.}
%     \label{tab:results}
% \end{table}
% We observe that our tensor method performs significantly better than the baseline. Preliminary results on the SPECT medical dataset analyzed in ~\cite{zhen2021community} also suggests that our method outperforms TENSOR-SCORE~\cite{ke2019community} and hypergraph Laplacian~\cite{ghoshdastidar2017consistency} approaches.


% \subsubsection{Centrality}

% \subsection{Experiments on real datasets}

% In this subsection we present some empirical centrality results on real-life datasets. In particular, we examine the similarities and differences between the rankings induced by Z-, H- and clique eigenvector centralities on the DAWN, tags-ask-ubuntu, and NDC-substances datasets\cite{Amburg-2020-categorical, Benson-2018-simplicial}.
% \begin{figure}
%     \centering
%     \scalebox{0.5}{\includegraphics[left]{figs/DAWN-3-kendalltaurankcorr.png}\includegraphics[left]{figs/DAWN-4-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/DAWN-5-kendalltaurankcorr.png}\includegraphics[left]{figs/DAWN-6-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/DAWN-7-kendalltaurankcorr.png}}
%     \caption{Kendall's $\tau_B$ rank correlation coefficient for the three centralities on the DAWN dataset. }
%     \label{fig:kendall_dawn}
% \end{figure}

% \begin{figure}
%     \centering
%     \scalebox{0.5}{\includegraphics[left]{figs/tags-ask-ubuntu-3-kendalltaurankcorr.png}\includegraphics[left]{figs/tags-ask-ubuntu-4-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/tags-ask-ubuntu-5-kendalltaurankcorr.png}\includegraphics[left]{figs/tags-ask-ubuntu-6-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/tags-ask-ubuntu-7-kendalltaurankcorr.png}}
%     \caption{Kendall's $\tau_B$ rank correlation coefficient for the three centralities on the ubuntu-tags dataset. Note that the last three plots are the same since the dataset contains hyperedges of size at most 5.}
    
%     \label{fig:kendall_tags}
% \end{figure}

% \begin{figure}
%     \centering
%     \scalebox{0.5}{\includegraphics[left]{figs/NDC-substances-3-kendalltaurankcorr.png}\includegraphics[left]{figs/NDC-substances-4-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/NDC-substances-5-kendalltaurankcorr.png}\includegraphics[left]{figs/NDC-substances-6-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/NDC-substances-7-kendalltaurankcorr.png}}
%     \caption{Kendall's $\tau_B$ rank correlation coefficient for the three centralities on the NDC-substances dataset.}
    
%     \label{fig:kendall_substances}
% \end{figure}

% \begin{figure}
%     \centering
%     \scalebox{0.5}{\includegraphics[left]{figs/congress-bills-3-kendalltaurankcorr.png}\includegraphics[left]{figs/congress-bills-4-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/congress-bills-5-kendalltaurankcorr.png}\includegraphics[left]{figs/congress-bills-6-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/congress-bills-7-kendalltaurankcorr.png}}
%     \caption{Kendall's $\tau_B$ rank correlation coefficient for the three centralities on the congress-bills dataset.}
    
%     \label{fig:kendall_bills}
% \end{figure}




% In Figures~\ref{fig:kendall_dawn}, ~\ref{fig:kendall_tags}, ~\ref{fig:kendall_substances}, and~\ref{fig:kendall_bills} we see that the adjusted-for-ties Kendall's $\tau_B$ rank correlation coefficient among the centrality measures varies substantially, indicating that the rankings provide complementary information.


==> clustering-cooking-and-dawn.tex <==
\subsection{Clustering}\label{subsec:clustering}

Our \ttsv\ algorithms also enable computation of hypergraph tensor embeddings, which may then serve as features for many clustering algorithms, such as $k$-means. Following this approach, we aim to embed the hypergraph adjacency tensor $\A$ in $\R^{n\times q}$, where $q$ is the target embedding dimension, so that each node is represented by a $q$-dimensional vector. We perform the embedding by finding a symmetric CP-decomposition~\cite{hitchcock1927expression,kolda2015numerical} of $\A$, meaning we seek an $n\times q$ matrix $\Mx{E}$ and a vector $\Vc{\lambda}\in \R^q$ such that the tensor norm given by 
\begin{equation}f(\Vc{\lambda},\Mx{E})=||\A-\T{X}||\mbox{ with }\T{X}=\sum_{j=1}^{q}\Vc{\lambda}_j\Mx{E}_j^{\otimes r}\label{eqn:objective}\end{equation}
is minimized, where $\Mx{E}=[\Mx{E}_1 \Mx{E}_2 \cdots \Mx{E}_q]$ and $\Mx{E}_j^{\otimes r}$ is the $r$-way tensor outer product of $\Mx{E}_j$ with itself. To optimize Equation~\ref{eqn:objective}, we employ a standard first-order optimization scheme and utilize the  closed-form expressions \cite{kolda2015numerical} for the gradients
\begin{align*}
\frac{\partial f}{\partial \Vc{\lambda}_j} &= -2\left[\A\Mx{E}_j^r-\sum_{k=1}^q\Vc{\lambda}_k\langle \Mx{E}_j,\Mx{E}_k\rangle ^r\right],\\
\frac{\partial f}{\partial \Mx{E}_j} &= -2d\Vc{\lambda}_j\left[\A\Mx{E}_j^{r-1}-\sum_{k=1}^q\Vc{\lambda}_k\langle \Mx{E}_j,\Mx{E}_k\rangle ^{r-1}\Mx{E}_k\right],
\end{align*}
where $\langle \Mx{E}_j,\Mx{E}_k\rangle=\Mx{E}_j^T\Mx{E}_k$, $\A\Mx{E}_j^r=\sum_{i_1=1}^n\cdots\sum_{i_r=1}^n\A_{i_1,\dots,i_r}\prod_{k=1}^r\Mx{E}_{j_{i_k}}$ is the \ttsv\ operation which results in a scalar.
%, and $\A\Mx{E}_j^{r-1}\in\R^n$ is the \ttsv[1] operation given by 
% \[
% \left[\A\Mx{E}_j^{r-1}\right]_{i_1}=\sum_{i_2=1}^n\cdots\sum_{i_r=1}^n\A_{i_1,\dots,i_r}\prod_{k=2}^r\Mx{E}_{j_{i_k}}.
% \]
 Note the \ttsv\ value is obtained from the \ttsv[1] vector simply by taking an inner product with $\Mx{E}_j.$ In the first order scheme, computing $f$ and its derivatives explicitly requires $O(qn^r)$ time, but we use \hyperref[alg:TTSV1G]{\ttsvG[1]}, together with the gradient computation approach outlined in~\cite{sherman2020estimating}, to cut this time down to $O(\ttsv[1]+ nq^2)$, where $O(\ttsv[1])$ is the worst-case runtime of \hyperref[alg:TTSV1G]{\ttsvG[1]}. After obtaining this CP decomposition for $\A$, the resulting embedding $E\in\R^{n\times q}$ may be used as features for a standard $k$-means clustering algorithm~\cite{hartigan1979algorithm} or more generally within any metric-space clustering framework. 
 %where $k$ is the desired number of clusters. 
%In practice, the value of $k$ is chosen to correspond to the number of ground truth clusters whenever such information is available. The pipeline is presented in Figure~\ref{fig:clustering}. 
% Beyond just $k$-means, the aforementioned embedding method is compatible with any metric-space clustering framework. 
\begin{figure}
    \centering
    \begin{tabular}{cc}
        \subfloat[\scriptsize t-SNE of embedding for the normalized Laplacian of the clique expansion (left) vs.~normalized Laplacian tensor of the hypergraph (right) of \texttt{cooking} \label{fig:tsne-cooking}]{\includegraphics[width=0.23\linewidth]{figs/tsne-zhou-cooking-r9-q10-degfrac0.2.pdf}\includegraphics[width=0.23\linewidth]{figs/tsne-cooking-r9-q10-degfrac0.2.pdf}} &  \subfloat[\scriptsize t-SNE of embedding for the normalized Laplacian of the clique expansion (left) vs.~normalized Laplacian tensor of the hypergraph (right) for \texttt{DAWN} \label{fig:tsne-DAWN}]{\includegraphics[width=0.23\linewidth]{figs/tsne-zhou-DAWN-r5-q20-degfrac0.2.pdf}\includegraphics[width=0.23\linewidth]{figs/tsne-DAWN-r5-q20-degfrac0.2.pdf}}
    \end{tabular}
    \caption{Comparison of matrix~\cite{zhou2006learning} to tensor embedding of \texttt{cooking} (left) and \texttt{DAWN} (right).}
    \label{fig:global_measures}
\end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width = 0.49\textwidth]{figs/DAWN.pdf}
%     \includegraphics[width = 0.49\textwidth]{figs/cooking.pdf}
%     \caption{t-SNE visualization of the tensor embedding for the contact-primary and cooking dataset. \sga{What if you did t-SNE plot of clustering based on the clique expansion? Would the clusters not be as well separated?}} %We observe that the clusters are well-separated.}
%     \label{fig:tsne}
% \end{figure}
Instead of clustering $\A$ directly, we cluster the corresponding normalized laplacian tensor $\LL$ from \cite{BANERJEE201714}, given by
\[
\LL_{p_1\dots p_{r}}=\begin{cases}-\left[\prod_{j=1}^{r}d(v_{p_j})^{-1/r}\right]\frac{\lvert e\rvert}{\lvert \beta(e)\rvert}&\mbox{ if } p_1\dots p_r \in \beta(e) \\
1 &\mbox{ if } p_1 = p_2 = \cdots = p_r \\
0 &\mbox{ otherwise}
\end{cases},
\]
It is worth noting that $\LL$ does not equally weight all blowups of an edge, and so \hyperref[alg:TTSV1gen]{\ttsvG} can not be directly applied.  However, if $d$ is the vector of all degrees we have that $\LL x^r = I x^r - \A (d^{[-\nicefrac{1}{r}]} \odot x)^r$ and, more generally, $\LL x^{r-k} = I x^{r-1} - \paren{d^{[-\nicefrac{1}{r}]}}^{\otimes k} \odot \A (d^{[-\nicefrac{1}{r}]} \odot x)^{r-k},$ where $\odot$ is the appropriate element-wise (Hadamard) tensor product.

We now apply the aforementioned clustering approach to \texttt{cooking} and \texttt{DAWN}. To better reveal clusters, we filter out high-degree nodes that appear in more that 20\% of the hyperedges. Figures~\ref{fig:tsne-cooking} and~\ref{fig:tsne-DAWN} present t-SNE~\cite{van2008visualizing} plots visualizing embeddings of these datasets. We color nodes based on hyperedge type metadata, assigning each node to the majority color of hyperedge it appears in.  
For each dataset, the left visualization presents the matrix-based embedding using the normalized Laplacian \cite{chung1997spectral} of the hypergraph's clique expansion graph, while the right shows the normalized Laplacian tensor embedding of the hypergraph.
%t-SNE of the normalized Laplacian embedding for the clique expansion matrix (left) and hypergraph tensor (right)
%The left of each figure shows a visualization of an unweighted version of the matrix-based embedding from~\cite{zhou2006learning}, while the right shows the same using our tensor approach. 
%\color{blue} That we observe well-separated clusters, provides qualitative evidence that the tensor embedding of $\A$ is able to distinguish communities. In fact, our tensor-based approach leads to better cluster separation in cooking. \color{black}
% We demonstrate that our approach is able to detect community structure in the t-SNE plots below. Note that the clusters are well-separated, implying a good embedding to distinguish communities.
%\sga{Perhaps replace with a simpler ``they are different" statement like we discussed: For both datasets, we observe starkly different geometry in their t-SNE plots when comparing the matrix versus tensor embeddings, providing qualitative evidence these approaches provide different information for clustering hypergraph data in practice.}  %In the tensor embedding for cooking and DAWN exhibit striations, whereas }
For both datasets we observe starkly different geometry between the t-SNE representations of the matrix and tensor embeddings, providing qualitative evidence that these two approaches are capturing different features of the hypergraph cluster in practice\footnote{We note that no effort was made to tune the performance of either clustring algorithm or evaluate which clustering is ``better."  Indeed, the understanding of which structure features of the hypergraph are highlighted by the CP-decomposition of $\LL$ is an interesting open question and is the source of potential future work.}. 




% \begin{figure}[h]
%     \centering
%     \scalebox{0.80}{\input{ttsv.tex}}
%     \caption{A graphical representation of TTSV for an order 3 tensor $A$.}
%     \label{fig:ttsv}
% \end{figure}


% While we employ $k$-means to perform the clustering, our embedding method is compatible with any metric-space clustering framework.
% \begin{figure}[h]
%     \centering
%     \scalebox{0.80}{\input{clustering.tex}}
%     \caption{A visualization of our clustering framework for nonuniform hypergraphs.}
%     \label{fig:clustering}
% \end{figure}

% \newpage


% \begin{figure}[h]
%     \centering
%     \resizebox{\columnwidth}{!}{\input{centrality.tex}}
%     \caption{A visualization of our centrality framework for nonuniform hypergraphs. \sga{Very nice figure idea, but should be redone to fix several cosmetic issues: (1) equations should be centered and either all above or all below the arrows, (2) consider shortening the names to acroymns (e.g. Z-eigen ventrality is just ZEC), (3) use tensor font for $\A$, (4) TTSVOB1 should just be TTSV1, consistent with rest of paper  } \sga{Also, I am confused here that this diagram shows us forming the banerjee tensor. I thought the whole point was we don't ``encode as a tensor" and instead do implicit TTSV}}
%     \label{fig:centrality}
% \end{figure}




% \begin{algorithm}[H]
% % \SetLine
% \SetKwRepeat{Repeat}{repeat}{until}
% \KwData{rank $r$ hypergraph $H=(V,E)$, tolerance $\tau$, step size $h$}
% \KwResult{Z-eigenvector centrality, $\Vc{x}$}
% $\Vc{y}=\frac{1}{|V|} \Vc{1}$\;

% \Repeat{$\frac{\max \Vc{g} - \min \Vc{g}}{\min \Vc{g}}<\tau$}{
% $\Vc{d} = \mbox{dominant eigenvector of TTSV2}((V,E),\Vc{y})$\;

% $\Vc{x} = \Vc{y}+h\cdot(\Vc{d}-\Vc{y})$\;

% $\Vc{g}=\Vc{x}\oslash \Vc{y}, \ \Vc{y} = \Vc{x}$\;
% }
% \Return{$\Vc{x}$}
% \caption{BG algorithm for computing Z-eigenvector centrality}
% \end{algorithm}

% \xhdr{Scalable generalized H-eigenvector centrality}

% The NQI power-like algorithm commonly used to compute H-eigenvector centrality relies on TTSV1 as the workhorse for each iteration~\cite{ng2010finding}. The algorithm is presented below.

% \begin{algorithm}[H]
% % \SetLine
% \KwData{rank $r$ hypergraph $H=(V,E)$, tolerance $\tau$}
% \KwResult{H-eigenvector centrality, \Vc{x}}
% $\Vc{y}=\frac{1}{|V|} \Vc{1}$\;

% $\Vc{z}=$ TTSV1($H,\Vc{y}$)\;

% \Repeat{$\lambda_{\max} -\lambda_{\min} < \tau$}
% {
% $\Vc{x}=\Vc{z}^{\nicefrac{1}{m-1}} / ||\Vc{z}^{\nicefrac{1}{m-1}}||_1$\;

% $\Vc{z}=$ TTSV1($H,\Vc{x}$)\;

% $\lambda_{\min}, \ \lambda_{\max} = \min{(\Vc{z} \oslash \Vc{x}^{m-1})}, \ \max{(\Vc{z} \oslash \Vc{x}^{m-1})}$
% }

% %converged = false\;

% % \For{$k$ in 0:iterations}{
% % $x_{k+1}=y_{k}^{1/(m-1)}/||y_{k}^{1/(m-1)}||_1$\;
% % $y_{k+1}=$ TTSV1($A,x^{k+1}$)\;
% % $\underline{\lambda}_{k+1}=\min_i\frac{[y_{k+1}]_i}{[x_{k+1}]_{i}^{m-1}}$\Comment{Compute lower estimate of eigenvalue}\;
% % $\bar{\lambda}_{k+1}=\max_i\frac{[y_{k+1}]_i}{[x_{k+1}]_{i}^{m-1}}$\Comment{Compute upper estimate of eigenvalue}\;
% % converged = $\bar{\lambda}_{k+1}-\underline{\lambda}_{k+1} <$ tolerance\;
% % \If{\mbox{converged}}{break}
% % }
% \Return{$\Vc{x}$}
% \caption{NQI algorithm for computing H-eigenvector centrality}
% \end{algorithm}
% \subsection{Clique expansion eigenvector centrality of general (weighted) hypergraphs}
% This centrality measure was first introduced in~\cite{benson2019three} in the uniform case. The nonuniform case was first presented in~\cite{amburg2021planted}, but was not analyzed there as it acted solely as a baseline to compare against. Here, we present the details of clique eigenvector centrality and analyze it. In particular, we show that it is stable and continuous in the notion of~\cite{segarra2015stability} as we change the weighting scheme. Furthermore, we show that the measure changes little when a hyperedge is added to ``unimportant'' nodes. Even when it is added to important nodes, we obtain a bound for the change in terms of their importances. These results are afforded by being able to apply the richly developed matrix eigenvector theory, which is either not possible or has not yet been developed in the case of matrices.

% \xhdr{Clique expansion eigevector centrality} Given a hypergraph $G,$ define its $n\times m$ weighted incidence matrix $I$ by writing $I_{v,e}=w_e$ if node $v$ appears in edge $e$ and $0$ otherwise. It is well-known that the clique adjacency matrix $$W=\sqrt{I}\sqrt{I^T}-D_V$$ where $D_V$ is a diagonal matrix with the weighted node degrees on its main diagonal corresponds to the adjacency matrix of a ``projected graph'' where $$W_{i,j}= \mbox{\# of times nodes $i$ and $j$ appear together in a hyperedge weighted by hyperedge weight}$$
% and the square root is taken componentwise.
% The clique eigenvector centrality vector $c$ is then the leading eigenvector of the system $$Wc=\lambda c.$$ In this formulation, a node is central if its neighbors are central in the weighted projected clique graph.

% \xhdr{Clique expansion eigenvector centrality is stable and continuous} Let us define the notions of stability and continuity that we use here.
% \begin{definition}
% A centrality measure $C$ is \textbf{stable} if given a vertex set $V$ and a set of hyperedges $E$ defined on it, given any two weighted hypergraphs $G$ and $H$ with those vertex and edge sets, we have $$|C^G(v)-C^H(v)|\leq K_G d(G,H)$$ for every node $v\in v$, where $C^G(v)$ is the centrality of node $v$ in G, $C^H(v)$ is its centrality in $H$, $K_G$ is a constand that depends on $G$, and $d(G,H)=\sum_{u,v}|W_G[u,v]-W_H[u,v]|$ is the weighted ``distance'' between the hypergraphs.

% \end{definition}

% \begin{definition}

% Given a weighted hypergraph $G$ on node set $V$ and edge set $E$ that has a projected graph incidence matrix $W_G$, define another matrix $W_\epsilon$ that has the same zero structure as $W_G$ so that $W_G+W_{\epsilon}\geq 0$, consider the weighted hypergraph $H$ on $(V,E)$ such that its projected graph incidence matrix is $W_G+W_\epsilon$. Then $C$ is a \textbf{continuous} centrality if $C^H(v)\to C^G(v)$ as $||W_\epsilon||_1\to 0$ for every node $v\in V$.

% \end{definition}

% The stability and continuity of clique expansion eigenvector centrality follows from the following theorem.

% \begin{theorem}

% Clique expansion eigenvector centrality for general hypergraphs is stable and continuous.
% \end{theorem}

% \begin{proof}
% Given two weighed hypergraphs $G$ and $H$ that are defined on the same node set, we know that changing the hyperedge weights will not affect the zero pattern of the corresponding projected graph adjacency matrices $W_G$ and $W_H$. By Proposition 4 in~\cite{segarra2015stability} the clique eigenvector centrality is stable, and by Proposition 6 it must also be continuous.

% \end{proof}

% % \xhdr{Perturbations in the unweighted case}
% % We want to quantify by how much any given component of the clique eigenvector centrality can change if we introduce one hyperedge. The following theorem will allow us to make these conclusions.
% % \begin{theorem}\label{thm:bound}
% % Given an unweighted hypergraph $G=(V,E),$ suppose that its clique expansion eigenvector centrality is $v$ with corresponding leading eigenvalue $\lambda$. If we include an additional hyperedge $h=\{i_1,\dots,i_k\}$ then the new eigenvector centrality vector $v'$ satisfies  $$\min_{s=\pm 1}||v-v'||_\infty\leq 8||v||_\infty\frac{\eta^2}{\lambda^2}+2\omega\frac{\mu}{\lambda}+4\omega\sqrt{k-1}\frac{\eta}{\lambda^2}$$
% % where $\eta^2=\sum_{l=1}^{k}\left[\sum_{j\in h\setminus\{i_l\}}v_j\right]^2,$ $\mu=\max_{l=1,\dots,k}\sum_{j\in h\setminus\{i_l\}}v_j$, and $\omega=||I-vv^T||_\infty$.
% % \end{theorem}
% % \begin{proof}

% % Suppose that the clique expansion adjacency matrix of the hyperedge is $A$. Then by the main theorem in~\cite{damle2020uniform} we know that $$\min_{s=\pm 1}||v-v'||_\infty\leq 8||v||_\infty\frac{||Av||_2^2}{\lambda^2}+2\omega \frac{||Av||_\infty}{\lambda}+4\frac{||Av||_2}{\lambda^2}\max_i||A[i,:]||_2$$
% % so it remains to show that $||Av||_2=\eta$ and $||Av||_\infty=\mu$ and $\max_i||A[i,:]||_2=\sqrt{k-1}$. The last statement follows since each vertex in the clique subgraph corresponding to $A$ has degree $(k-1)$. The first and middle statements follow since $A[l,j]v_j$ is nonzero and equal to $v_j$ precisely at indexes $j\in h\setminus \{i_l\}$ for every $l\in\{1,\dots,k\}$. This concludes the proof.
% % \end{proof}

% % The formulation in the preceeding theorem allows us to get an intuition for what factors will make the increase potentially large. The following corollary shows that The componentwise change is greatest when the nodes in $h$ are ``important'' in terms of the values in $v$ and least when the nodes are not important.

% % \begin{coro}

% % The upper bound in Theorem~\ref{thm:bound} is maximized when the nodes in $h$ correspond to the indexes of components in $v$ having the greatest values while it is minimized if they correspond to components having the smallest values in $v$.
% % \end{coro}

% % \begin{proof}

% % This is clear since $\eta$ is a sum of squares of sums of the positive components of $v$ corresponding to the nodes in $h$ while $\mu$ is a maximum over sums of those same components.
% % \end{proof}

% \subsection{Tensor eigenvector centrality detects higher-order information}
% Here, we present a case study on a synthetic dataset that demonstrates that $H$- and $Z$- tensor eigenvectors are able to distinguish higher-order patterns that standard graph projection methods are incapable of detecting. In particular, we consider two hypergraphs, $G_A$ and $G_B$ seen in the figure below. $G_A$ and $G_B$ both have the same clique expansions, and the clique expansions of their line graphs are also the same. In particular, if $A$ is the node-hyperedge incidence matrix of $G_A$ and $B$ is the same for $G_B,$ then $W=A^TA=B^TB$ and $W'=AA^T=BB^T.$ These kinds of hypergraphs are refered to as gram mates~\cite{everett2013dual,kirkland2018two,kim2022gram}. Since all graph projection approaches work on either $W$ or $W'$, the two hypergraphs are rendered indistinguishable under this approach, meaning, foe example, the resulting clique expansion eigenvector centralities are the same. However, we show that the corresponding $H$- and $Z$-eigenvector centralities \textit{do} distinguish the the two hypergraphs, producing meaningfully different centrality vectors.


% \section{Experiments}
% Here, we conduct two suites of experiments that demonstrate the usefulness of our methods and their superiority to baselines. The first suite shows that our methods perform orders of magnitude faster on both synthetic and real-life datasets. The second suite showcases results for two applications: clustering and centrality of the underlying hypergraph. In particular, we demonstrate the superiority of our clustering scheme to other tensor-based methods, and highlight the effectiveness of our tensor-eigenvector-based centralities in finding meaningfully-different rankings of nodes.


% \subsection{Performance on random hypergraphs}

% \xhdr{A hypergraph stochastic block model}
% Here, we describe a simple hypergraph generation scheme which we use to test the ability of our method to recover ground truth assignment in the stochastic setting, with the presence of noise. We randomly partition $n$ nodes into $k$ clusters. We form hyperedges on nodes within clusters with probability $q$. We form edges across clusters with probability $p$. The maximum hyperedge size $r$ is also taken as a parameter. If we want, we can choose $q=1-p$ to reduce the dimensionality.

% \subsection{Tensor operation run times}
% Here, we present runtime experiments on synthetic and real-life hypergraphs demonstrating the superiority of our approach to existing methods and baselines.
% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{figs/ttsv1-times}
%     \caption{Speedup factors of the generating-function-based algorithm for TTSV1 vs. the combinations-based, naive baseline, and explicit sparse tensor baseline. Missing times indicate that a) the combinations-based or naive baseline algorithms timed out after 1 hour or b) the explicit tensor baseline algorithm forced an out-of-memory error.}
%     \label{fig:ttsv1_time}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{figs/ttsv2-times}
%     \caption{Speedup factors of the generating-function-based algorithm for TTSV2 vs. the combinations-based, naive baseline, and explicit sparse tensor baseline. Missing times indicate that a) the combinations-based or naive baseline algorithms timed out after 1 hour or b) the explicit tensor baseline algorithm forced an out-of-memory error.}
%     \label{fig:ttsv1_time}
% \end{figure}
% \subsection{Applications}

% \subsubsection{Clustering}
% \xhdr{Results on real-life datasets}
% We test the performance of the algorithm by comparing against a spectral method followed by $k$-means on the projected graph corresponding to the hypergraph. We test performance on two real-world datasets:

% 1) Yelp Madison~\cite{amburg2020hypergraph}, where hyperedges connect reviewers who wrote reviews of restaurants of a given cuisine over the course of a month and node labels correspond to the majority review category; 2) Amazon blues~\cite{amburg2020hypergraph}, where hyperedges connect reviewers of products who wrote reviews in a given subgenre of vinyl blues records over the course of a month and node labels correspond to the majority review category.
% %and 3) SPECT~\cite{zhen2021community}, where hyperedges connect patients who share the same categorical features and node labels correspond to the presence or absence of a cardiovascular disease.
% We use the scaled hamming distance~\cite{zhen2021community} between the ground truth node labels and the clustering to compare across methods, the performance of which is noted in Table~\ref{tab:results}.

% \begin{table}[h]
%     \centering
%     % \begin{tabular}{c|ccc}
%     %      dataset & $r\leq$&tensor error  &projected error\\
%     %      \hline
%     %     Yelp Madison & 3&  \textbf{0.138}& 0.144\\
%     %     Amazon blues & 3 & \textbf{0.284}& 0.321
        
%     % \end{tabular}
%     \begin{tabular}{c|ccc}
%          dataset & $r\leq$&tensor NMI  &projected NMI\\
%          \hline
%         madison-restaurant-reviews & 3&  \textbf{0.166}& 0.095\\
%         vegas-bars-reviews & 5&  \textbf{0.235}& 0.092\\
%         DAWN & 3 & \textbf{0.672} & 0.582
%         % Amazon blues & 3 & \textbf{0.284}& 0.321
        
%     \end{tabular}

%     \caption{Performance of the tensor-based algorithm vs. a spectral clustering baseline. We report the filtering parameter $r$ that resulted in the best performance increase.}
%     \label{tab:results}
% \end{table}
% We observe that our tensor method performs significantly better than the baseline. Preliminary results on the SPECT medical dataset analyzed in ~\cite{zhen2021community} also suggests that our method outperforms TENSOR-SCORE~\cite{ke2019community} and hypergraph Laplacian~\cite{ghoshdastidar2017consistency} approaches.


% \subsubsection{Centrality}

% \subsection{Experiments on real datasets}

% In this subsection we present some empirical centrality results on real-life datasets. In particular, we examine the similarities and differences between the rankings induced by Z-, H- and clique eigenvector centralities on the DAWN, tags-ask-ubuntu, and NDC-substances datasets\cite{Amburg-2020-categorical, Benson-2018-simplicial}.
% \begin{figure}
%     \centering
%     \scalebox{0.5}{\includegraphics[left]{figs/DAWN-3-kendalltaurankcorr.png}\includegraphics[left]{figs/DAWN-4-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/DAWN-5-kendalltaurankcorr.png}\includegraphics[left]{figs/DAWN-6-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/DAWN-7-kendalltaurankcorr.png}}
%     \caption{Kendall's $\tau_B$ rank correlation coefficient for the three centralities on the DAWN dataset. }
%     \label{fig:kendall_dawn}
% \end{figure}

% \begin{figure}
%     \centering
%     \scalebox{0.5}{\includegraphics[left]{figs/tags-ask-ubuntu-3-kendalltaurankcorr.png}\includegraphics[left]{figs/tags-ask-ubuntu-4-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/tags-ask-ubuntu-5-kendalltaurankcorr.png}\includegraphics[left]{figs/tags-ask-ubuntu-6-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/tags-ask-ubuntu-7-kendalltaurankcorr.png}}
%     \caption{Kendall's $\tau_B$ rank correlation coefficient for the three centralities on the ubuntu-tags dataset. Note that the last three plots are the same since the dataset contains hyperedges of size at most 5.}
    
%     \label{fig:kendall_tags}
% \end{figure}

% \begin{figure}
%     \centering
%     \scalebox{0.5}{\includegraphics[left]{figs/NDC-substances-3-kendalltaurankcorr.png}\includegraphics[left]{figs/NDC-substances-4-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/NDC-substances-5-kendalltaurankcorr.png}\includegraphics[left]{figs/NDC-substances-6-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/NDC-substances-7-kendalltaurankcorr.png}}
%     \caption{Kendall's $\tau_B$ rank correlation coefficient for the three centralities on the NDC-substances dataset.}
    
%     \label{fig:kendall_substances}
% \end{figure}

% \begin{figure}
%     \centering
%     \scalebox{0.5}{\includegraphics[left]{figs/congress-bills-3-kendalltaurankcorr.png}\includegraphics[left]{figs/congress-bills-4-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/congress-bills-5-kendalltaurankcorr.png}\includegraphics[left]{figs/congress-bills-6-kendalltaurankcorr.png}}\newline\scalebox{0.5}{ \includegraphics[left]{figs/congress-bills-7-kendalltaurankcorr.png}}
%     \caption{Kendall's $\tau_B$ rank correlation coefficient for the three centralities on the congress-bills dataset.}
    
%     \label{fig:kendall_bills}
% \end{figure}




% In Figures~\ref{fig:kendall_dawn}, ~\ref{fig:kendall_tags}, ~\ref{fig:kendall_substances}, and~\ref{fig:kendall_bills} we see that the adjusted-for-ties Kendall's $\tau_B$ rank correlation coefficient among the centrality measures varies substantially, indicating that the rankings provide complementary information.


==> generating-functions.tex <==
\subsection{Generating function approach} \phantom{}\newline
\stephen{ start with the inner loop as the bulk of the computational time, think through what happens with a small edge, then this leads naturally to the generating function approach }\sga{This exposition is nice}\newline
It is clear that the bulk of the time in both Algorithm~\ref{alg:TTSV1} and \ref{alg:TTSV2} is spent in the inner-most loop, iteratating over the elements of $\kappa(e)$ for all edges $e$.  Indeed, for most real world data sets, where the size of a typical edge is much smaller than the largest edge, this is a significant bottleneck as the size of the this set scales exponentially with the size of the edge, i.e.\ $\size{\kappa(e)} = \bigOh{r^{\size{e}}}$.  However, by taking a generating function approach the inner loop can be considerably simplified and accelerated.  To illustrate this, consider the 
summation over the inner loop for the case when $e = \set{u,v} \in E(v))$,
\begin{align*}
    \sum_{x \in \kappa(\set{u,v})} w_e \frac{\phi_1(x,v)}{\Vc{b}_v} \prod_{i \in x} \Vc{b}_i &= \frac{w_e}{\Vc{b}_v} \sum_{k_u = 1}^{r-1} \phi_1( u^{k_u} v^{r - k_u}, v) \Vc{b}_u^{k_u} \Vc{b}_v^{r-k_u} \\
    &= w_e \sum_{k_u = 1}^{r-1} \frac{(r-1)!}{k_u! (r-1-k_u)!} \Vc{b}_u^{k_u}\Vc{b}_v^{r-1-k_u} \\
    &= w_e (r-1)! \sum_{k_u = 1}^{r-1} \frac{1}{k_u!} \Vc{b}_u^{k_u} \frac{1}{(r-1-k_u)!} \Vc{b}_v^{r-1-k_u}. \tag{\textasteriskcentered}\label{eq:sum}
\end{align*}
We note that the summation in (\ref{eq:sum}) can be viewed as a convolution of two sequences 
\[ 0,\frac{1}{1!}\Vc{b}_u^1, \frac{1}{2!}\Vc{b}_u^2, \ldots, \frac{1}{(r-1)!} \Vc{b}_u^{r-1} \quad \textrm{and} \quad \frac{1}{0!} \Vc{b}_v^0, \frac{1}{1!}\Vc{b}_v^1,  \frac{1}{2!}\Vc{b}_v^2, \ldots, \frac{1}{(r-1)!}\Vc{b}_v^{r-1}.\]
Alternatively, if we define $u_r(t) = \sum_{k=1}^{r-1} \frac{1}{k!}\Vc{b}_u^kt^k$ and $v_r(t) = \sum_{k=0}^{r-1} \frac{1}{k!}\Vc{b}_v^kt^k$, the summation (\ref{eq:sum}) may be thought of as the coefficient of $t^{r-1}$ in $u_r(t)v_r(t)$, which we will denote $(u_r(t)v_r(t))[t^{r-1}]$. 
In fact, we have that for any $d\geq 0$ the summation is equal to $\paren{u_{r+d}(t) v_{r+d}(t)}[t^{r-1}]$ and thus taking 
\[ u(t) = \sum_{k=1}^{\infty} \frac{1}{k!}\Vc{b}_u^k = e^{\Vc{b}_ut} - 1 \quad \textrm{and} \quad v(t) = \sum_{k=0}^{\infty} \frac{1}{k!} \Vc{b}_v^k = e^{\Vc{b}_vt},\] we have that $(u(t)v(t))[t^{r-1}]$ is the value of the inner sum for an arbitrary choice of largest edge size $r$. Extending the above argument to an arbitrary edge $e \in E(v)$, we have that the inner sum in Algorithm \ref{alg:TTSV1} is given by \[w_e (r-1)!\paren{e^{\Vc{b}_vt} \prod_{u \in e - \set{v}} \paren{e^{\Vc{b}_ut} - 1 }}[t^{r-1}].\] A similar approach can be taken for TTSV2, yielding Algorithms \ref{alg:TTSV1gen} and \ref{alg:TTSV2gen}.


\begin{figure}
\centering
\begin{minipage}[t]{0.9\linewidth}
  \vspace{0pt}  
  \begin{algorithm}[H] %\small
  \LinesNotNumbered 
 %\SetLine
\KwData{rank $r$ hypergraph $(V,E,w)$, vector $\Vc{b}$}
\KwResult{$\A\Vc{b}^{r-1}=\Vc{s}$}
\For{$v\in V$}{
$c \gets 0$\;

\For{$e\in E(v)$}{
$c\pluseq \displaystyle w_e (r-1)! \paren{e^{\Vc{b}_vt} \prod_{ \substack{ u \in e \\ u \neq v}}(e^{\Vc{b}_ut} -1)}[t^{r-1}]$\;
}
$\Vc{s}_v \gets  c$\;
}
\Return{$\Vc{s}$}
\caption{Implicit TTSV1 via generating functions\ilya{$e$ is overloaded for hyperedge and $\exp$.}}
\label{alg:TTSV1gen}
\end{algorithm}
\end{minipage} \\
    \begin{minipage}[t]{0.9\linewidth}
\begin{algorithm}[H] %\small
\LinesNotNumbered 
\KwData{rank $r$ hypergraph $(V,E)$, vector $\Vc{b}$}
\KwResult{$\A \Vc{b}^{r-2}=\Mx{Y}$}
\For{$(u,v)\in V^2$ with $u\leq v$}{
$c \gets 0$\;

\For{$e\in E(u,v)$}{
\If{$u = v$}{
$c\pluseq \displaystyle w_e (r-2)! \paren{e^{\Vc{b}_ut} \prod_{ \substack{ x \in e \\ x \neq u}}(e^{\Vc{b}_ut} -1)}[t^{r-2}]$\;
}
\Else{
$c\pluseq \displaystyle w_e (r-2)! \paren{e^{(\Vc{b}_u + \Vc{b}_v)t} \prod_{ \substack{ x \in e \\ u \neq u,v}}(e^{\Vc{b}_ut} -1)}[t^{r-2}]$\;
}
$\Mx{Y}_{uv} \gets  c$\;
}
}
\Return{$\Mx{Y}+\Mx{Y}^T-\mathrm{diag}(\Mx{Y})$}
\caption{Implicit TTSV2 via generating functions}
\label{alg:TTSV2gen}
\end{algorithm}
\end{minipage}
\caption{Implicit TTSV1 (top) and TTSV2 (bottom) for the hypergraph adjacency tensor $\A$ via the generating function approach.}
\end{figure}

While this generating function simplifies the exposition of these algorithms, without an efficient means of extracting the appropriate coefficient from the generating function this framework is of little practical use.  \stephen{this transitions sucks}. \sga{I think it is fine. I added ``Accordingly" :-)}  Accordingly, we present two different options for evaluating the generating function approach, a subset expansion approach which runs in time $\bigOh{\paren{\size{e} + \log_2(r)}2^{\size{e}}}$, and a modification of Karatsuba algorithm for multiplication which runs in time $\bigOh{\size{e} r^{\log_2(3)}}$.  We note that the subset expansion approach is asymptotically faster for $\size{e} < \log_2(3) \log_2(r)$ and for larger edges the Karatsuba algorithm is more efficient.  Thus, if we assume the subset algorithm is only used for sufficiently small edges, its running time is $\bigOh{\log(r)2^{\size{e}}}$. \stephen{This section could probably be expanded a bit} \sga{With what? Seems complete to me but could be missing something.}


\begin{figure}
\begin{minipage}[t]{0.44\linewidth}
  \vspace{0pt}  
  \begin{algorithm}[H] \small
  \LinesNotNumbered 
 %\SetLine
\KwData{degree $d$ polynomials $f(t)$ and $g(t)$}
\KwResult{$f(t) g(t)$} \\
\phantom{  } $d' \gets \displaystyle\floor{\frac{d}{2}}$\; \\
$f_0 \gets \displaystyle\sum_{j=0}^{d'} f[t^j]t^j$\; \\
$f_1 \gets \displaystyle\sum_{j=0}^{d-d'} f[t^{j+d'}]t^j$\; \\
 $g_0 \gets \displaystyle\sum_{j=0}^{d'} g[t^j]t^j$\; \\
 $g_1 \gets \displaystyle\sum_{j=0}^{d-d'} g[t^{j+d'}]t^j$\; \\
$z_2 \gets \textsc{Karatsuba}(f_1,g_1,d-d')$\; \\
 $z_1 \gets \textsc{Karatsuba}(f_0+f_1 ,g_0+g_1 ,\ceil{\frac{d}{2}} )$\\
$z_0 \gets \textsc{Karatsuba}(f_0,g_0,d')$\\
\Return{$z_2 t^{2d'} + (z_1 - z_0 - z_2) t^{d'} + z_0 $}
\caption{\textsc{Karatsuba} Karatsuba multiplication}
\label{alg:Karatsuba}
\end{algorithm}
\end{minipage} \hfil
\begin{minipage}[t]{0.50\linewidth}
 \vspace{0pt}
\begin{algorithm}[H] \small
\LinesNotNumbered 
\KwData{$a, b_1, \ldots, b_k \in \R$ and $r \in \N$.}
\KwResult{$\paren{e^{at} \prod_i \paren{e^{b_it} - 1}}[t^r]$}
$f \gets \sum_{j=0}^r \frac{a^j}{j!} t^j$\;\\
\For{ $i = 1, \ldots, k$}{
$g \gets \sum_{j=1}^r \frac{b_i^j}{j!}t^j$ \; 

$f \gets \textsc{Karatsuba}(f,g,r)$\; 

$f \gets \sum_{j=0}^r f[t^j] t^j$\; 
}
\Return{$f[t^r]$}
\caption{Karatsuba evaluation of generating function}
\label{alg:Kartsub_gen}
\end{algorithm}
\vspace{-6mm}
\begin{algorithm}[H]
    \small
    \LinesNotNumbered
    \KwData{$a,b_1,\ldots,b_k \in \R$ and $r \in \N$}
    \KwResult{$\paren{e^{at} \prod_i \paren{e^{b_it} - 1}}[t^r]$}
    $c \gets 0$\; \\
    \For{ S \in 2^{[k]}}{
        $c \pluseq (-1)^{k - \size{S}} \paren{a + \sum_{s \in S} b_s }^r$\;
    }
    \Return{ \nicefrac{c}{r!}}
    \caption{Subset enumeration evaluation of generating function}  
    \label{alg:subset_gen}
    \end{algorithm}
\end{minipage}
\caption{Subalgorithms for the Karatsuba and subset enumeration approaches to evaluate generating functions \sga{Flop order as per Stephen}}\label{fig:algs}
\end{figure}

% \begin{figure}
%     \centering
%     \begin{algorithm}[H]
%     \small
%     \LinesNotNumbered
%     \KwData{$a,b_1,\ldots,b_k \in \R$ and $r \in \N$}
%     \KwResult{$\paren{e^{at} \prod_i \paren{e^{b_it} - 1}}[t^r]$}
%     $c \gets 0$\; \\
%     \For{ S \in 2^{[k]}}{
%         $c \pluseq (-1)^{k - \size{S}} \paren{a + \sum_{s \in S} b_s }^r$\;
%     }
%     \Return{ \nicefrac{c}{r!}}
%     \caption{Subset enumeration evaluation of generating function}  
%     \label{alg:subset_gen}
%     \end{algorithm}
    

% \end{figure}

\begin{proposition}\label{P:TTSVgen}
Let $H$ be a rank $r$ hypergraph with $m$ edges, let $\delta = \frac{\Vol{H}}{m}$, and let $k^*$ \sga{Would be nice if we put that approximate form you mentioned here, like $k^* \approx 1.234...$} be the solution to \[ 2^k \log_2(r) = k r^{\log_2(3)}.\]  The implicit TTSV1 via generating functions algorithm  (Algorithm \ref{alg:TTSV1gen}) runs in time at least 
\[ \begin{cases} \bigOmega{\Vol(H)2^{\delta}\log_2(r)} & \delta < \frac{1}{2}k^* \\ \bigOmega{\Vol(H)2^{(1-\lilOh{1})\delta}\log_2(r)} & \frac{1}{2} k^* \leq \delta \leq k^*  \\
\bigOmega{\Vol(H)\delta r^{\log_2(3)}} & k^* < \delta
\end{cases} \]
and at most  
\[\bigOh{\log_2(r)m\frac{r-\delta}{r-2} + r^{2+\log_2(3)}m\frac{\delta-2}{r-2}}.\]
Similarly, the implicit TTSV2 via generating functions algorithm (Algorithm \ref{alg:TTSV2gen}) runs in time at least
\[ \begin{cases} \bigOmega{\Vol(H)\delta 2^{\delta}\log_2(r)} & \delta < \frac{1}{2}k^* \\ \bigOmega{\Vol(H)\delta 2^{(1-\lilOh{1})\delta}\log_2(r)} & \frac{1}{2} k^* \leq \delta \leq k^*  \\
\bigOmega{\Vol(H)\delta^2 r^{\log_2(3)}} & k^* < \delta
\end{cases} \]
and at most  
\[\bigOh{\log_2(r)\Vol(H)\frac{r-\delta}{r-2} + r^{2+\log_2(3)}\Vol(H)\frac{\delta-2}{r-2}}.\]
\end{proposition}

\begin{proof}
As in the proof of Proposition \ref{P:TTSV}, the run times of Algorithm \ref{alg:TTSV1gen} and \ref{alg:TTSV2gen} both depend on the sequence of edges sizes of the hypergraph, yielding  
\[ \bigTheta{\sum_{e \in E} \size{e} h(\size{e},r-1)} \qaud \textrm{and} \quad \bigTheta{\sum_{e \in E} \paren{\frac{\size{e^2}+\size{e}}{2}}h(\size{e},r-1)}, \]
respectively, where $h(k,r)$ is the run time of extracting the coefficient of $t^{r-1}$ in the generating function associated with an edge of size $k$. If for every edge, we use the faster of the Karatsuba algorithm and the subset expansion algorithm, this gives that 
\[ h(k,r) = \bigTheta{\min \set{ \log_2(r)2^k, k r^{\log_2(3)}}}.\]

In order to understand the growth rate of the run times it is important to separate out the edges which are treated with the Karatsuba algorithm and those treated with the subset expansion approach.  To that end, we focus first on those edges for which the generating function is evaluated by the subset expansion approach and denote by $e_S$ and $m_S$ the average size and number of such edges, respectively.  We note that if $ k < \ell$, then
\[ k 2^k + \ell 2^{\ell} -  (k+1)2^{k+1} - (\ell-1)2^{\ell-1} = (\ell+1)2^{\ell-1} -  (k+2)2^k \geq 0. \] 
Thus the run time of for the subset selection approach is minimized when all $m_S$ of the edges have size $e_S$, and maximized when all the edges have either size $2$ or size $k^*$. In particular, this means that we may assume the maximum run time occurs when the only edges which use the subset expansion approach are size 2.  Thus if the $m_k$ is the number of edges of size $k^*$ which maximizes the run time, then the maximum run time is  

\begin{center}
\begin{multiline}
8\log_2(r) \frac{rm -(r-k^*)m_k - \Vol(H) }{r-2}+ (k^*)^2 r^{\log_2(3)} m_k +r^{2+\log_2(3)} \frac{\Vol(H) - (k^*-2)m_k - 2m}{r-2}.
\end{multiline}
\end{center}



As the coefficient on $m_k$ in this expression is 0, the overall runtime is maximized when the only edge sizes present are $2$ and $r$. Noting that $\Vol(H) = 2m + \delta m$ yields the claimed  maximum run time of
\[ \bigTheta{\log_2(r)m\frac{r-\delta}{r-2} + r^{2+\log_2(3)}m\frac{\delta-2}{r-2}}. \]

To address the minimum run time, we recall that by standard results the contribution of the run time of all edges of size at least $k^*$ is minimized when their sizes are equal.  Similarly, we showed above that the contribution to the run time of all edges with size at most $k^*$ is minimized when their sizes are equal.  Thus, if we define $V_S$ and $m_S$ as the number and volume of edges which are processed by the subset expansion, and similarly define $m_K$ and $V_K$ for the edges processed by the Karatsuba method, the asymptotic run time is given by
\[ V_S 2^{\frac{V_S}{m_S}}\log_2(r) + m_K \paren{\frac{V_K}{m_K}}^2r^{\log_2(3)} = V_S 2^{\frac{V_S}{m_S}}\log_2(r) + \frac{V_K^2}{m_K}r^{\log_2(3)}. \]



Letting $\delta_S$ and $\delta_K$ be the average size of edge processed by the subset expansion method and that Karatsuba method, respectively, i.e.\ $\delta_S = \nicefrac{V_S}{m_S}$ and $\delta_K = \nicefrac{V_K}{m_K}$, this can be rewritten as 
\[ V_S 2^{\delta_S}\log_2(r) + V_K \delta_K r^{\log_2(3)}.\] 

Now suppose that $V_K \geq \epsilon \Vol(H)$ for some fixed $\epsilon > 0$.  Then, as $\delta_K \geq \delta$, we that 
\[ \frac{V_K \delta_K r^{\log_2(3)}}{\Vol(H) \delta r^{\log_2(3)}} \in \bigOmega{1}.\]
In particular, this implies that the only case where the run-time is $\lilOh{\Vol(H)\delta r^{\log_2(3)}}$ is when $V_S = (1-\lilOh{1}) \Vol(H)$ and $\delta_S = (1-\lilOh{1)}\delta$. As $\delta_S < k^*$, this implies that if $\delta \geq k^*$, then the minimal run time is $\bigOmega{\Vol(H)\delta}$.

  We note that we may view $V_S$ and $V_K$ as functions of $\delta_S$ and $\delta_K$, yielding
\[ f(\delta_S,\delta_K) = \frac{m\delta_K - \Vol(H)}{\delta_K - \delta_S}\delta_S 2^{\delta_s}\log_2(r) + \frac{\Vol(H) - m\delta_S}{\delta_K - \delta_S}\delta_K^2 r^{\log_2(3)}.\]

It is a straightforward, albeit tedious exercise, to show that, taken as a function of $\delta_K$, $f$ is minimized when $d_K$ takes the value 
\[ \delta_K^* = \delta_S + \delta_S\sqrt{1 - \frac{2^{\delta_S}\log(r)}{\delta_S r^{\log_2(3)}}} \leq 2\delta_S.\]
In particular, this implies that if $\delta_S < \frac{1}{2}k^*$  (or equivalently, if $\delta < k^*$) then the minimum run time is 
\[\bigTheta{ \Vol(H) 2^{\delta}\log_2(r)}.\]

The analysis for Algorithm \ref{alg:TTSV2gen} follows similar lines.
\end{proof}
\sga{This was a difficult proof, thanks! I wonder if there is something slightly more sloppy but simple we could put here to help the reader unpack the Big Oh complexities. I don't yet know exactly what that is, but maybe we could impose a few reasonable assumptions: ``assume that average hyperedge cardinality is $\delta=\log(m)$, etc. Then...". In general, it would be lovely if we could say ``We improve $O(n^r)$ to something that looks roughly like BLANK" -- and I don't know what BLANK is yet. }

==> xx.tex <==



==> xxs.tex <==


